Delay-Adaptive Learning in Generalized Linear Contextual Bandits

In this paper, we consider online learning in generalized linear contextual bandits where rewards are not immediately observed. Instead, rewards are available to the decision-maker only after some delay, which is unknown and stochastic. We study the performance of two well-known algorithms adapted to this delayed setting: one based on upper confidence bounds, and the other based on Thompson sampling. We describe modifications on how these two algorithms should be adapted to handle delays and give regret characterizations for both algorithms. Our results contribute to the broad landscape of contextual bandits literature by establishing that both algorithms can be made to be robust to delays, thereby helping clarify and reaffirm the empirical success of these two algorithms, which are widely deployed in modern recommendation engines.

==> heavy_decay_extension.tex <==

{\color{red}
\section{Extensions: Delays with first moment}\label{sec:heavy_decay_extension}



In Assumption \ref{delay}, we assume decays are at-most as heavy as exponential distributions. In deed, this is the minimum assumption to guarantee the leading term in the regrets (Eqn. \eqref{Rt} and Eqn. \eqref{Rt_Bayes}) does not depend on delay-related parameters.

In this section, we relax the assumption on delays in Assumption \ref{delay} and only require the boundedness of  the first moment of delays. In this case, the leading term in the regret will depend on delay-related parameters.

\begin{assumption}\label{ass:delays_2}
Assume $\{D_t\}_{t=1}^T$ are independent non-negative random variables and there exists a constant $B>0$ such that $\mathbb{E}[D_t]\leq B$ for all $t=1,2,\cdots,T$. Further assume there exists a constant $M>0$ and a distribution $\xi$ with mean $\mu < B$ such that
for any  $m \geq M$ and  $t \in [T]$,
\[
\P(D_t \geq m) \leq \P(D \geq m),
\]
where  $D \sim \xi$.
\end{assumption}
\begin{proposition}\label{prop:weak_G}
Under Assumption \ref{ass:delays_2}, with probability $1-\delta$,
\[
G_T^* \leq (M+B)+\log \left(\frac{T}{\delta}\right) +\sqrt{2(M+B)\log\left(\frac{T}{\delta}\right)},
\]
where $G_T^* = \max_{1\leq t\leq T} {G_t}$.
\end{proposition}

\begin{proof}{Proof of Proposition \ref{prop:weak_G}.}
\begin{eqnarray}\label{G_expecation}
\mathbb{E}[G_t] = \mathbb{E}\left[\sum_{s=1}^{t-1}\mathbb{I}\{s+D_s \geq t\}\right] = \sum_{s=1}^{t-1}\mathbb{P}(s-D_s \ge t) = \sum_{s=1}^{t-2}\mathbb{P}(s-D_s > t) \leq M+B.
\end{eqnarray}
And similarly,
\begin{eqnarray}\label{G_variance}
\mathbb{V}[G_t] = \mathbb{V}\left[\sum_{s=1}^{t-1}\mathbb{I}\{s+D_s \geq t\}\right] \leq \sum_{s=1}^{t-1}\mathbb{P}(s-D_s \ge t) = \sum_{s=1}^{t-2}\mathbb{P}(s-D_s > t) \leq M+B.
\end{eqnarray}

By Bernstein's inequality, for any $0< \delta <1$ and any $t$ we have, with probability at least $1-\delta$,
\[
G_t -\E[G_t] \leq \log(\frac{1}{\delta}) +\sqrt{2\V[G_t]\log\left(\frac{1}{\delta}\right)}
\]
Applying the union bound and combined with \eqref{G_expecation}-\eqref{G_variance}, we have  with probability at least $1-\delta$,
\[
\max_{1\leq t\leq T} {G_t}- (M+B) \leq \log \left(\frac{T}{\delta}\right) +\sqrt{2(M+B)\log\left(\frac{T}{\delta}\right)}.
\]
\end{proof}



\begin{theorem}\label{thm: UCBregret_first_moment}
Assume Assumptions \ref{a1} and \ref{ass:delays_2}.  Fix any $\delta$. There exists a universal constant $C:=C(C_1,C_2,M,\mu,\sigma_0,\hat{\sigma},\,\sigma,\kappa)>0$, such that if we run DUCB-GLCB with $\tau := C \left(d+\log(\frac{1}{\delta})\right)$ and $\beta_t = \frac{\hat{\sigma}}{\kappa} \sqrt{\frac{d}{2} \log \left(1+\frac{2(t-G_t)}{d}\right)+\log(\frac{1}{\delta})}+G_t$, then, with probability at least $1-5\delta$, the regret of the algorithm is upper bounded by
\begin{eqnarray}\label{Rt_first_moment}
R_T
 &\leq& \tau + L_{g} \left( 2\left(\sqrt{M+B}+\sqrt{\log \left(\frac{T}{\delta}\right) }+\left({2(M+B)\log\left(\frac{T}{\delta}\right)}\right)^{1/4}\right)\sqrt{2T d \log \left(\frac{T}{d}\right)} + \frac{2d \hat{\sigma}}{\kappa} \log\left(\frac{T}{d\delta}\right)\sqrt{T}\right).
\end{eqnarray} \end{theorem}
It is easy to check that, in this case,
\begin{eqnarray}\label{Rt_order_first_moment}
R_T =O \left(d\sqrt{T}\log({T})+\sqrt{M+B}\sqrt{Td\log(T)}+\sqrt{Td}\log(T)+(M+B)^{1/4}\sqrt{Td}(\log(T))^{3/4}\right).
\end{eqnarray} 
\begin{theorem}\label{alg:BayesRegret_first_moment}
Assume Assumptions \ref{a1} and \ref{ass:delays_2}. There exists a universal constant $C:=C(C_1,C_2,M,\mu,\sigma_0,\sigma_G,\,\sigma,\kappa)>0$, such that if we run exploration with $\tau := C \left(d+\log(\frac{1}{\delta})\right)$,
\begin{eqnarray}\label{Rt_Bayes}
R^B_T(\pi_{\tau}^{\text{PS}}) 
=O \left(d\sqrt{T}\log({T})+\sqrt{M+B}\sqrt{Td\log(T)}+\sqrt{Td}\log(T)+(M+B)^{1/4}\sqrt{Td}(\log(T))^{3/4}\right)
\end{eqnarray}
\end{theorem}
}









